What does guidance do? A fine-grained analysis in a simple setting

The use of guidance in diffusion models was originally motivated by the premise that the guidance-modified score is that of the data distribution tilted by a conditional likelihood raised to some power. In this work we clarify this misconception by rigorously proving that guidance fails to sample from the intended tilted distribution. Our main result is to give a fine-grained characterization of the dynamics of guidance in two cases, (1) mixtures of compactly supported distributions and (2) mixtures of Gaussians, which reflect salient properties of guidance that manifest on real-world data. In both cases, we prove that as the guidance parameter increases, the guided model samples more heavily from the boundary of the support of the conditional distribution. We also prove that for any nonzero level of score estimation error, sufficiently large guidance will result in sampling away from the support, theoretically justifying the empirical finding that large guidance results in distorted generations. In addition to verifying these results empirically in synthetic settings, we also show how our theoretical insights can offer useful prescriptions for practical deployment.

==> files/mixture-uniforms-body.tex <==
\section{Mixture of uniform distributions}
\label{sec:pre_uniform}

Here we provide some intuition for our main result on mixtures of uniform distributions, i.e. the case when $\Pone$ and $\Pmone$ are supported on $[\alpha_1, \alpha_2]$ and $[-\alpha_2, -\alpha_1]$, respectively, $0<\alpha_1<\alpha_2$. 

We make the following assumption on $\Pone$ and $\Pmone$:
\begin{assumption}\label{pre_assump:ratio}
    We assume the densities $\Pone, \Pmone$ have $\ratio$-bounded densities with respect to each other for some $\ratio \geq 1$. Namely $\forall x_1 \in (-\alpha_2, - \alpha_1), x_2\in (\alpha_1,  \alpha_2)$: $\frac{1}{\ratio} \leq \frac{\Pmone(x_1)}{\Pone(x_2)} \leq \ratio$.
\end{assumption}

Under Assumption~\ref{pre_assump:ratio} we show that running guidance leads most of the mass of the initial Gaussian to concentrate at the edge of $\Pone$. In particular, we prove the following Theorem.


\begin{theorem}[Convergence to the edge of the support]\label{pre_thm:convergencecompact}
    Assume $\frac{\ln(w)}{16\sqrt w} \leq \frac{\alpha_1\alpha_2}{\beta}$, $\alpha_2^2 \leq \ln(w)$. Then running the guided ODE with parameter $w$ for the mixture model $p$ defined in~\eqref{e:mm} under Assumption~\ref{assump:ratio}, with probability at least $1 - e^{-\frac{w\alpha_1^2}{512\ratio^2}}$, the resulting sample $\xs(1)$ is in $\pa{\alpha_2\bigl(1-\frac{32}{\sqrt{\ln(w)}}\bigr),  \alpha_2}$.
    %at least $1-e^{-w^2/2}$ concentrates in the interval $(1-O(1/\sqrt{\ln(w)} , 1)$ at the end.
\end{theorem}

The formal proof of Theorem~\ref{pre_thm:convergencecompact} which combines all the pieces that we present in this section appears in the supplement.
%%
In high level, we show that the particle goes through two major phases: first, if we have the condition that the initial point $x(0)$ satisfies $\Omega(-\sqrt w)$, %\jlnotes{why is the initial point $\Omega(-\sqrt{w})$?} 
it goes far from the support of the distributions on the positive direction up to order $\Theta(w)$. Then, in the second phase, it comes back to the support of $\Pone$ but by the time it reaches the support it is already close to the end of the process; in particular, we show that it cannot move too much on the support of $\Pone$ once it arrives there. Hence the particle gets stuck near the edge of the support.

To simplify the notation, for all $t\in [0,T]$, denote the random variable $a_t x + \xi_t$ by $X_t$ (observe that $X_0 = x$). Then, it is easy to check that the score at time $t$ can be obtained from the posterior mean of $X_0$ given $X_t$. $\nabla \log(p_t(\yy))= a_t\E[\Xvar - \yy| \Yvar=\yy]$, and $\nabla \log(p_t(\yy|z=\pm 1)) = a_t \E[\Xvar - \yy| \Yvar=\yy, z=\pm 1]$.

We denote $\E[\Xvar | \Yvar=\yy]$ in short by $\E[\Xvar | \yy]$ and $\E[\Xvar | \Yvar=\yy, z=\pm 1]$ in short by $\E[\Xvar | \yy, z=\pm 1]$. 
We additionally consider the change of variable $s(t) \triangleq a_t = e^{t-T}$ and its corresponding inverse function $t(s) = \ln(s) + T$, and $\xs(s) = x(t(s))$, where $s$ varies in the interval $[\sinit, 1]$ for $\sinit = e^{-T}$.
Define the following conditional probabilities of the two components, conditioned on $\Yvar$: $\pright = \Prr{z=1| \Yvar = x(t)}$ and $\pleft = \Prr{z=-1| \Yvar = x(t)}$.
We now present a key algebraic manipulation of the probability flow ODE in~\eqref{eq:odeform} which enables us to estimate it more effectively:

\begin{lemma}[Alternative view on probability flow ODE]
    The probability flow ODE can be written as
    \begin{align}
    x'(t) &= \frac{1}{b_t^2}\pa{a_t\E[\Xvar | x(t), z=1] - a_t^2 x(t)} \\
    &\qquad +\frac{w}{b_t^2}\pleft\pa{a_t\E[ \Xvar | x(t), z=1] - a_t\E[ \Xvar | x(t), z=-1]},\label{eq:pre_keyform}
\end{align}
or with respect to $\xs(s)$ in variable $s$:
\begin{align}
    \xs'(s) &= \frac{1}{b_t^2}\pa{\E[\Xvar | \xs(s), z=1] - a_t \xs(s)} \\
    &\qquad +\frac{w}{b_t^2}\pleft\pa{\E[ \Xvar | \xs(s), z=1] - \E[ \Xvar | \xs(s), z=-1]}\,.\label{eq:pre_keyform2}
\end{align}
\end{lemma}


\paragraph{\textbf{High level sketch of proof of Theorem~\ref{pre_thm:convergencecompact}}}

The details for the proof are quite involved, so due to space constraints here we can only describe a roadmap for the full argument that is provided in the supplement. Note that the second term in~\eqref{eq:pre_keyform} $\frac{w}{b_t^2}\pleft\pa{\E[ \Xvar | x(t), z=1] - \E[ \Xvar | x(t), z=-1]}$ is a positive dominant term (compared to the first term) unless we have $\pleft = O(1/w)$, which happens only when $x(t) = \Omega(\ln(w))$. First, we show that (1) starting from a high probability region of initial point, $x(t)$ will get to $x(t) \geq \Omega(\ln(w))$ at some point, using the dominance of the second term in Lemma~\ref{lem:firstphase}. Then, in the case where $x(t_0) = \Omega(\ln(w))$ for some time $t_0$, (2) we show a lower bound on the time that it takes for $x(t)$ to get back to the proximity of the origin and then an upper bound on how much it can move inside the support in Lemma~\ref{lem:secondphase}. Finally in Lemma~\ref{lem:convtosupport} we show that $x(t)$ does converge to the interval under the probability event of Lemma~\ref{lem:firstphase}. Building upon these Lemmas, we prove the final result in Theorem~\ref{pre_thm:convergencecompact}.

==> formatting.tex <==
\renewcommand{\thesection}{\arabic{section}}

==> theorems_with_boxes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%Theorem styles
\newtheoremstyle{norm}
{12pt}
{12pt}
{}
{}
{\bf}
{:}
{.5em}
{}

\newtheorem{thm}{Theorem}[section]
\newtheorem*{thm*}{Theorem}
\newtheorem{clm}[thm]{Claim}
\newtheorem*{clm*}{Claim}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem*{conj*}{Conjecture}
%\newtheorem{cons}{Construction}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem*{lem*}{Lemma}

\theoremstyle{norm}
\newtheorem{prb}[thm]{Problem}%[section]
\newtheorem*{prb*}{Problem}

\newtheorem{alg}[thm]{Algorithm}
\newtheorem{assm}[thm]{Assumption}
\newtheorem{ax}[thm]{Axiom}
\newtheorem*{ax*}{Axiom}
\newtheorem{df}[thm]{Definition}
\newtheorem*{df*}{Definition}
\newtheorem{ex}[thm]{Example}
\newtheorem*{ex*}{Example}
\newtheorem{exr}[thm]{Exercise}
\newtheorem{expl}[thm]{Exploration}%prb
\newtheorem{fct}[thm]{Fact}
\newtheorem{mdl}[thm]{Model}
\newtheorem{pos}[thm]{Postulate}
\newtheorem*{pos*}{Postulate}
%\newtheorem{sprb}{Problem}%numbering for solutions
\newtheorem{pr}[thm]{Proposition}
\newtheorem*{pr*}{Proposition}
\newtheorem{qu}[thm]{Question}
\newtheorem*{qu*}{Question}
\newtheorem{rem}[thm]{Remark}
\newtheorem*{rem*}{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%DEFINING BOX COMMANDS
\newcommand{\prbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [prbox] (box){
\begin{minipage}[l]{6in}
#1
\end{minipage}
};
\end{tikzpicture}\\%
}
}
\newcommand{\prbbox}[1]{\prbox{\begin{prb}#1\end{prb}}}
\newcommand{\expbox}[1]{\prbox{\begin{expl}#1\end{expl}}}
\newcommand{\sprbbox}[1]{\prbox{\begin{sprb}#1\end{sprb}}}

\newcommand{\thbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [thbox] (box){
\begin{minipage}[l]{6in}
#1
\end{minipage}
};
\end{tikzpicture}\\%
}}
%6.68

\newcommand{\thmbox}[1]{\thbox{\begin{thm}#1\end{thm}}}
\newcommand{\dfbox}[1]{\thbox{\begin{df*}#1\end{df*}}}

\newcommand{\grbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [cpbox] (box){
\begin{minipage}[l]{6in}
#1
\end{minipage}
};
\end{tikzpicture}\\%
}}
\newcommand{\cpbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [cpbox] (box){
\begin{minipage}[c]{.2in}
%\hspace{-.2in}
%\dbend
\includegraphics[scale=0.35]{\filepath/key}
\end{minipage}
\begin{minipage}[t]{6in}%6.25
#1
\end{minipage}
};
\end{tikzpicture}\\%
}}


\newcommand{\wrbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [wrbox] (box){
\begin{minipage}[c]{.2in}
%\hspace{-.2in}
%\dbend
{\Huge \bf !}
\end{minipage}
\begin{minipage}[t]{6in}%6.25
#1
\end{minipage}
};
\end{tikzpicture}\\%
}}
\newcommand{\hintbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [hnbox] (box){
\begin{minipage}[l]{6in}
\textbf{Hint:} {#1}
\end{minipage}
};
\end{tikzpicture}\\%
}
}
%white box
\newcommand{\whbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [hnbox] (box){
\begin{minipage}[l]{6in}
{#1}
\end{minipage}
};
\end{tikzpicture}\\%
}
}
%6.68
%END DEFINING BOX COMMANDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Box commands
%\thbox{...} makes a theorem box
%\thmbox{...} makes a theorem box labeled "Theorem"
%\prbox{...} makes a problem box
%\prbbox{...} makes a problem box labeled "Problem"
%\cpbox{...} makes a concept box labeled "Concept"
%\wrbox{...} makes a warning box.
%\dfbox{...} makes a definition box (same as problem box) labeled "> Definition"
%\sprbbox{...} makes a problem box labeled "Problem" (use this when you're making a copy of a previous problem box to put the solution afterwards; it has a numbering system separate from problems).

 
% for testing purposes only
\usepackage[english]{babel} 
\usepackage{blindtext} 
%%%%%%%%
%begin doc
%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%DEFINING THE BOXES.
% Problem box (simple box, blue)
\tikzstyle{prbox} = [draw=black, fill=blue!20, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
% Theorem box (double border, gray)
\tikzstyle{thbox} = [draw=black,double, fill=blue!10, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
%\tikzstyle{fancytitle} =[fill=red, text=white]
% Concept box (shadowed, light green)
\tikzstyle{cpbox} = [drop shadow={
    shadow scale=1}, draw=black, fill=green!10, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
\tikzstyle{wrbox} = [drop shadow={
    shadow scale=1}, draw=black, fill=yellow!10, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
\tikzstyle{hnbox} = [draw=black, fill=white, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
%END DEFINING BOXES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

